Estimating Causal Effects With Partial Covariates For Clinical Interpretability

Estimating the causal effects of an intervention in the presence of confounding is a frequently occurring problem in applications such as medicine. The task is challenging since there may be multiple confounding factors, some of which may be missing, and inferences must be made from high-dimensional, noisy measurements. In this paper, we propose a decision-theoretic approach to estimate the causal effects of interventions where a subset of the covariates is unavailable for some patients during testing. Our approach uses the information bottleneck principle to perform a discrete, low-dimensional sufficient reduction of the covariate data to estimate a distribution over confounders. In doing so, we can estimate the causal effect of an intervention where only partial covariate information is available. Our results on a causal inference benchmark and a real application for treating sepsis show that our method achieves state-of-the-art performance, without sacrificing interpretability.

==> conclusion.tex <==
\section{Conclusion}
\label{conclusion}

We have presented a novel approach to estimate causal relationships with respect to incomplete covariates from an decision-theoretic point of view. For this purpose, we analysed the role of a sufficient covariate in the context of the IB framework to estimate the causal effect. By introducing a discrete latent space, we can estimate the causal effect if parts of the covariates are missing during test time, while accounting for both measured and hidden confounders. In contrast to previous methods, the compression parameter $\lambda$ in the IB framework allows for a task-dependent adjustment of the latent dimensionality. Directions for future work include modelling structured hidden confounders as well as adopting CEIB to implicit generative models.

==> foundations.tex <==
\section{Preliminaries and Related Work}
\label{sec:related_work}

\paragraph{Potential Outcomes and Counterfactual Reasoning} Counterfactual reasoning (CR) has drawn large attention, particularly in the medical community. Counterfactual models are essentially rooted in causal inference and may be used to determine the causal effects of an intervention. These models are formalised in terms of \emph{potential outcomes} \citep{Neyman23,splawa1990application,rubin1978bayesian}. Assume we have two choices of taking a treatment $t$, and not taking a treatment (control) $c$. Let $Y_t$ denote the outcomes under $t$ and $Y_c$ denote outcomes under the control $c$. The counterfactual approach assumes that there is a pre-existing joint distribution $P(Y_t, Y_c)$ over outcomes. This joint distribution is hidden since $t$ and $c$ cannot be applied simultaneously.  Applying an action $t$ thus only reveals $Y_t$, but not $Y_c$. In this setting, computing the effect of an intervention involves computing the difference between when an intervention is made and when no treatment is applied \citep{pearl2009causality, morgan2015counterfactuals}. We would subsequently choose to treat with $t$ if, 
\begin{align}
\mathbb{E}[L(Y_t)] \leq \mathbb{E}[L(Y_c)] 
\end{align}
for loss $L$ over $Y_t$ and $Y_c$ respectively. Potential outcomes are typically applied to cross-sectional data \citep{NIPS2017_6767,DBLP:conf/nips/2017/SchulamS17} and sequential time settings. Notable examples of models for counterfactual reasoning include \citet{JohanssonTAR} and \citet{bottou2013counterfactual}. Specifically, \citet{JohanssonTAR} propose a neural network architecture called TARnet to estimate the effects of interventions. Similarly, Gaussian Process CR (GPCR) models are proposed in \citet{NIPS2017_6767, DBLP:conf/nips/2017/SchulamS17} and further extended to the multitask setting in \citet{AlaaS17}.  Off-policy evaluation methods in reinforcement learning (RL) offer another perspective for reasoning about counterfactuals, and have been extensively explored to estimate the outcomes of a particular policy or series of treatments based on retrospective observational data (see for example \citet{dudik2011doubly}, \citet{thomas2016data},  \citet{jiang2016doubly}).  

Importantly, none of these approaches enable estimating treatment effects in the presence of confounding and partial covariate information. We emphasise that using the IB principle to perform causal inference in these settings is (to our knowledge) novel.

\paragraph{Decision-Theoretic View of Causal Inference} 
The decision theoretic approach to causal inference focuses on studying the \emph{effects of causes} rather than the causes of effects \citep{dawid07}. Here, the key question is \emph{what is the effect of the causal action on the outcome?} The outcome may be modelled as a random variable $Y$ for which we can set up a decision problem. That is, at each point, the value of $Y$ is dependent on whether $t$ or $c$ is selected. The decision-theoretic view of causal inference considers the distributions of outcomes given the treatment or control, $P_{t}$ and $P_{c}$ and explicitly computes an expected loss of $Y$ with respect to each action choice. Finally, the choice to treat with $t$ is made using Bayesian decision theory if,
\begin{align}
\mathbb{E}_{Y \sim P_t}[L(Y)] \leq \mathbb{E}_{Y \sim P_c}[L(Y)].
\end{align}
Thus in this setting, causal inference involves comparing the expected losses over the hypothetical distributions $P_t$ and $P_c$ for outcome $Y$.

\paragraph{Information Bottleneck}
The IB principle \citep{art:tishby:ib} describes an information theoretic approach which is used to compress a random variable $X$ with respect to a second random variable $Y$. The compression of $X$ is described by another random variable $Z$. Achieving an optimal compression requires solving the following problem,
\begin{align}
{\min}_{p(z|x)} I(X;Z) - \lambda I(Z;Y),
\label{eq:1}
\end{align}
under the assumption that $Y$ and $Z$ are conditionally independent given $X$. Here, $I$ represents the mutual information between two random variables and $\lambda$ controls the degree of compression.  In its classical form, the IB principle is defined only for discrete random variables. However, in recent years multiple IB relaxations for Gaussian \citep{art:chechik:gib} and meta-Gaussian variables \citep{mgib} have been proposed.

\paragraph{Deep Latent Variable Models} 
Deep latent variable models have recently received remarkable attention and been applied to a variety of problems. Among these, variational autoencoders (VAEs) employ the reparameterisation trick introduced in \citet{kingma2013auto, pmlr-v32-rezende14} to infer a variational approximation over the posterior distribution of the latent space $p(z|x)$.   Important work in this direction include \citet{KingmaSemi} and \citet{Jang}. Most closely related to the work we present here, is the application of VAEs in a healthcare setting by \citet{Louizos}. Here, the authors introduce a Cause-Effect VAE (CEVAE) to estimate the causal effect of an intervention in the presence of noisy proxies. 

Despite their differences, it has been shown that there are several close connections between the VAE framework and the IB principle. \citet{DVIB} introduce the Deep Information Bottleneck (DIB). This is essentially a VAE where $X$ is replaced by $Y$ in the decoder. In contrast, the approach in this paper considers the IB principle to perform \emph{causal inference} in scenarios where only \emph{partial covariate data} is available at test time. 


